Parameterized Hypercomplex Graph Neural Networks for Graph Classification

Despite recent advances in representation learning in hypercomplex (HC) space, this subject is still vastly unexplored in the context of graphs. Motivated by the complex and quaternion algebras, which have been found in several contexts to enable effective representation learning that inherently incorporates a weight-sharing mechanism, we develop graph neural networks that leverage the properties of hypercomplex feature transformation. In particular, in our proposed class of models, the multiplication rule specifying the algebra itself is inferred from the data during training. Given a fixed model architecture, we present empirical evidence that our proposed model incorporates a regularization effect, alleviating the risk of overfitting. We also show that for fixed model capacity, our proposed method outperforms its corresponding real-formulated GNN, providing additional confirmation for the enhanced expressivity of HC embeddings. Finally, we test our proposed hypercomplex GNN on several open graph benchmark datasets and show that our models reach state-of-the-art performance while consuming a much lower memory footprint with 70& fewer parameters. Our implementations are available at https://github.com/bayer-science-for-a-better-life/phc-gnn.

==> references.tex <==
@article{hamilton_quaternion,
 ISSN = {03027597},
 URL = {http://www.jstor.org/stable/20489494},
 author = {Wm. R. Hamilton},
 journal = {Proceedings of the Royal Irish Academy (1836-1869)},
 pages = {1--16},
 publisher = {Royal Irish Academy},
 title = {Theory of Quaternions},
 volume = {3},
 year = {1844}
}

@article{Wu_2021,
   title={A Comprehensive Survey on Graph Neural Networks},
   volume={32},
   ISSN={2162-2388},
   url={http://dx.doi.org/10.1109/TNNLS.2020.2978386},
   DOI={10.1109/tnnls.2020.2978386},
   number={1},
   journal={IEEE Transactions on Neural Networks and Learning Systems},
   publisher={Institute of Electrical and Electronics Engineers (IEEE)},
   author={Wu, Zonghan and Pan, Shirui and Chen, Fengwen and Long, Guodong and Zhang, Chengqi and Yu, Philip S.},
   year={2021},
   month={Jan},
   pages={4–24}
}

@InProceedings{mpnn_qm9, title = {Neural Message Passing for Quantum Chemistry}, author = {Justin Gilmer and Samuel S. Schoenholz and Patrick F. Riley and Oriol Vinyals and George E. Dahl}, pages = {1263--1272}, year = {2017}, editor = {Doina Precup and Yee Whye Teh}, volume = {70}, series = {Proceedings of Machine Learning Research}, address = {International Convention Centre, Sydney, Australia}, month = {06--11 Aug}, publisher = {PMLR}, pdf = {http://proceedings.mlr.press/v70/gilmer17a/gilmer17a.pdf}, url = {http://proceedings.mlr.press/v70/gilmer17a.html} }

@book{hc_numbers,
 ISBN={978-1-4612-8191-7},
 URL = {https://www.springer.com/gp/book/9781461281917},
 author = {Kantor, I.L.~and Solodovnikov, A.S.},
 publisher = {Springer-Verlag New York},
 title = {Hypercomplex Numbers},
 subtitle = {An Elementary Introduction to Algebras},
 year = {1989}
}



@misc{tay2019,
      title={Lightweight and Efficient Neural Natural Language Processing with Quaternion Networks}, 
      author={Yi Tay and Aston Zhang and Luu Anh Tuan and Jinfeng Rao and Shuai Zhang and Shuohang Wang and Jie Fu and Siu Cheung Hui},
      year={2019},
      eprint={1906.04393},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@article{ecfp4,
author = {Rogers, David and Hahn, Mathew},
title = {Extended-Connectivity Fingerprints},
journal = {Journal of Chemical Information and Modeling},
volume = {50},
number = {5},
pages = {742-754},
year = {2010},
doi = {10.1021/ci100050t},
    note ={PMID: 20426451},

URL = { 
        https://doi.org/10.1021/ci100050t
    
},
eprint = { 
        https://doi.org/10.1021/ci100050t
    
}

}

@misc{hu2020open,
      title={Open Graph Benchmark: Datasets for Machine Learning on Graphs}, 
      author={Weihua Hu and Matthias Fey and Marinka Zitnik and Yuxiao Dong and Hongyu Ren and Bowen Liu and Michele Catasta and Jure Leskovec},
      year={2020},
      eprint={2005.00687},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{dwivedi2020benchmarking,
      title={Benchmarking Graph Neural Networks}, 
      author={Vijay Prakash Dwivedi and Chaitanya K. Joshi and Thomas Laurent and Yoshua Bengio and Xavier Bresson},
      year={2020},
      eprint={2003.00982},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@InProceedings{Zhu_2018_ECCV,
author = {Zhu, Xuanyu and Xu, Yi and Xu, Hongteng and Chen, Changjian},
title = {Quaternion Convolutional Neural Networks},
booktitle = {Proceedings of the European Conference on Computer Vision (ECCV)},
month = {September},
year = {2018}
}

@article{Parcollet2019QuaternionCN,
  title={Quaternion Convolutional Neural Networks for Heterogeneous Image Processing},
  author={Titouan Parcollet and Mohamed Morchid and G. Linar{\`e}s},
  journal={ICASSP 2019 - 2019 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  year={2019},
  pages={8514-8518}
}

@inproceedings{
trabelsi2018deep,
title={Deep Complex Networks},
author={Chiheb Trabelsi and Olexa Bilaniuk and Ying Zhang and Dmitriy Serdyuk and Sandeep Subramanian and Joao Felipe Santos and Soroush Mehri and Negar Rostamzadeh and Yoshua Bengio and Christopher J Pal},
booktitle={International Conference on Learning Representations},
year={2018},
url={https://openreview.net/forum?id=H1T2hmZAb},
}

@INPROCEEDINGS{gaudet2018deep,
  author={C. J. {Gaudet} and A. S. {Maida}},
  booktitle={2018 International Joint Conference on Neural Networks (IJCNN)}, 
  title={Deep Quaternion Networks}, 
  year={2018},
  volume={},
  number={},
  pages={1-8},
  doi={10.1109/IJCNN.2018.8489651}}
  

@inproceedings{
parcollet2018quaternion,
title={Quaternion Recurrent Neural Networks},
author={Titouan Parcollet and Mirco Ravanelli and Mohamed Morchid and Georges Linarès and Chiheb Trabelsi and Renato De Mori and Yoshua Bengio},
booktitle={International Conference on Learning Representations},
year={2019},
url={https://openreview.net/forum?id=ByMHvs0cFQ},
}

@misc{nguyen2020quaternion,
      title={Quaternion Graph Neural Networks}, 
      author={Dai Quoc Nguyen and Tu Dinh Nguyen and Dinh Phung},
      year={2020},
      eprint={2008.05089},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{
zhang2021parameterization,
title={Parameterization of Hypercomplex Multiplications},
author={Aston Zhang and Yi Tay and SHUAI Zhang and Alvin Chan and Anh Tuan Luu and Siu Hui and Jie Fu},
booktitle={International Conference on Learning Representations},
year={2021},
url={https://openreview.net/forum?id=rcQdycl0zyk}
}
@inproceedings{
anonymous2021generalizing,
title={Generalizing Complex/Hyper-complex Convolutions to Vector Map Convolutions},
author={Anonymous},
booktitle={Submitted to International Conference on Learning Representations},
year={2021},
url={https://openreview.net/forum?id=K398CuAKVKB},
note={under review}
}

@inproceedings{
anonymous2021algebranets,
title={AlgebraNets},
author={Anonymous},
booktitle={Submitted to International Conference on Learning Representations},
year={2021},
url={https://openreview.net/forum?id=guEuB3FPcd},
note={under review}
}


@misc{anonymous,
  title= {Suppressed for Anonymity},
  author= {Author, N. N.},
  year= {2021}
}

@inproceedings{arjovsky2016unitary,
  title={Unitary evolution recurrent neural networks},
  author={Arjovsky, Martin and Shah, Amar and Bengio, Yoshua},
  booktitle={International Conference on Machine Learning},
  pages={1120--1128},
  year={2016}
}



@inproceedings{structure2vec,
author = {Dai, Hanjun and Dai, Bo and Song, Le},
title = {Discriminative Embeddings of Latent Variable Models for Structured Data},
year = {2016},
publisher = {JMLR.org},
abstract = {Kernel classifiers and regressors designed for structured data, such as sequences, trees and graphs, have significantly advanced a number of interdisciplinary areas such as computational biology and drug design. Typically, kernels are designed beforehand for a data type which either exploit statistics of the structures or make use of probabilistic generative models, and then a discriminative classifier is learned based on the kernels via convex optimization. However, such an elegant two-stage approach also limited kernel methods from scaling up to millions of data points, and exploiting discriminative information to learn feature representations.We propose, structure2vec, an effective and scalable approach for structured data representation based on the idea of embedding latent variable models into feature spaces, and learning such feature spaces using discriminative information. Interestingly, structure2vec extracts features by performing a sequence of function mappings in a way similar to graphical model inference procedures, such as mean field and belief propagation. In applications involving millions of data points, we showed that structure2vec runs 2 times faster, produces models which are 10, 000 times smaller, while at the same time achieving the state-of-the-art predictive performance.},
booktitle = {Proceedings of the 33rd International Conference on International Conference on Machine Learning - Volume 48},
pages = {2702–2711},
numpages = {10},
location = {New York, NY, USA},
series = {ICML'16}
}

@article{WL_test,
author = {Weisfeiler, B.~and Lehman A.A.},
title = {A reduction of a graph to a canonical form and an algebra arising during this reduction},
journal = {Nauchno-Technicheskaya Informatsia},
volume = {2(9)},
year = {1968},
pages = {12–16}
}

@Article{ADMET_floriane,
author = {Montanari, Floriane and Kuhnke, Lara and Ter Laak, Antonius and Clevert, Djork-Arn\'e},
title = {Modeling Physico-Chemical ADMET Endpoints with Multitask Graph Convolutional Networks},
journal = {Molecules},
volume = {25},
year = {2020},
number = {1}
}

@article{DBLP:journals/debu/HamiltonYL17,
  author    = {William L. Hamilton and
               Rex Ying and
               Jure Leskovec},
  title     = {Representation Learning on Graphs: Methods and Applications},
  journal   = {{IEEE} Data Eng. Bull.},
  volume    = {40},
  number    = {3},
  pages     = {52--74},
  year      = {2017},
  url       = {http://sites.computer.org/debull/A17sept/p52.pdf},
  timestamp = {Tue, 10 Mar 2020 16:23:49 +0100},
  biburl    = {https://dblp.org/rec/journals/debu/HamiltonYL17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{pmlr-v70-gilmer17a, title = {Neural Message Passing for Quantum Chemistry}, author = {Justin Gilmer and Samuel S. Schoenholz and Patrick F. Riley and Oriol Vinyals and George E. Dahl}, booktitle = {Proceedings of the 34th International Conference on Machine Learning}, pages = {1263--1272}, year = {2017}, editor = {Doina Precup and Yee Whye Teh}, volume = {70}, series = {Proceedings of Machine Learning Research}, address = {International Convention Centre, Sydney, Australia}, month = {06--11 Aug}, publisher = {PMLR}, pdf = {http://proceedings.mlr.press/v70/gilmer17a/gilmer17a.pdf}, url = {http://proceedings.mlr.press/v70/gilmer17a.html}, abstract = {Supervised learning on molecules has incredible potential to be useful in chemistry, drug discovery, and materials science. Luckily, several promising and closely related neural network models invariant to molecular symmetries have already been described in the literature. These models learn a message passing algorithm and aggregation procedure to compute a function of their entire input graph. At this point, the next step is to find a particularly effective variant of this general approach and apply it to chemical prediction benchmarks until we either solve them or reach the limits of the approach. In this paper, we reformulate existing models into a single common framework we call Message Passing Neural Networks (MPNNs) and explore additional novel variations within this framework. Using MPNNs we demonstrate state of the art results on an important molecular property prediction benchmark; these results are strong enough that we believe future work should focus on datasets with larger molecules or more accurate ground truth labels.} }

@inproceedings{
xu2018how,
title={How Powerful are Graph Neural Networks?},
author={Keyulu Xu and Weihua Hu and Jure Leskovec and Stefanie Jegelka},
booktitle={International Conference on Learning Representations},
year={2019},
url={https://openreview.net/forum?id=ryGs6iA5Km},
}

@inproceedings{
Hu*2020Strategies,
title={Strategies for Pre-training Graph Neural Networks},
author={Weihua Hu and Bowen Liu and Joseph Gomes and Marinka Zitnik and Percy Liang and Vijay Pande and Jure Leskovec},
booktitle={International Conference on Learning Representations},
year={2020},
url={https://openreview.net/forum?id=HJlWWJSFDH}
}

@InProceedings{pmlr-v80-xu18c, title = {Representation Learning on Graphs with Jumping Knowledge Networks}, author = {Xu, Keyulu and Li, Chengtao and Tian, Yonglong and Sonobe, Tomohiro and Kawarabayashi, Ken-ichi and Jegelka, Stefanie}, booktitle = {Proceedings of the 35th International Conference on Machine Learning}, pages = {5453--5462}, year = {2018}, editor = {Jennifer Dy and Andreas Krause}, volume = {80}, series = {Proceedings of Machine Learning Research}, address = {Stockholmsmässan, Stockholm Sweden}, month = {10--15 Jul}, publisher = {PMLR}, pdf = {http://proceedings.mlr.press/v80/xu18c/xu18c.pdf}, url = {http://proceedings.mlr.press/v80/xu18c.html}, abstract = {Recent deep learning approaches for representation learning on graphs follow a neighborhood aggregation procedure. We analyze some important properties of these models, and propose a strategy to overcome those. In particular, the range of "neighboring" nodes that a node’s representation draws from strongly depends on the graph structure, analogous to the spread of a random walk. To adapt to local neighborhood properties and tasks, we explore an architecture – jumping knowledge (JK) networks – that flexibly leverages, for each node, different neighborhood ranges to enable better structure-aware representation. In a number of experiments on social, bioinformatics and citation networks, we demonstrate that our model achieves state-of-the-art performance. Furthermore, combining the JK framework with models like Graph Convolutional Networks, GraphSAGE and Graph Attention Networks consistently improves those models’ performance.} }

@InProceedings{batchnorm_ioffe,
author = {Ioffe, Sergey and Szegedy, Christian},
title = {Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift},
year = {2015},
publisher = {JMLR.org},
abstract = {Training Deep Neural Networks is complicated by the fact that the distribution of each layer's inputs changes during training, as the parameters of the previous layers change. This slows down the training by requiring lower learning rates and careful parameter initialization, and makes it notoriously hard to train models with saturating nonlinearities. We refer to this phenomenon as internal covariate shift, and address the problem by normalizing layer inputs. Our method draws its strength from making normalization a part of the model architecture and performing the normalization for each training mini-batch. Batch Normalization allows us to use much higher learning rates and be less careful about initialization, and in some cases eliminates the need for Dropout. Applied to a state-of-the-art image classification model, Batch Normalization achieves the same accuracy with 14 times fewer training steps, and beats the original model by a significant margin. Using an ensemble of batch-normalized networks, we improve upon the best published result on ImageNet classification: reaching 4.82\% top-5 test error, exceeding the accuracy of human raters.},
booktitle = {Proceedings of the 32nd International Conference on International Conference on Machine Learning - Volume 37},
pages = {448–456},
numpages = {9},
location = {Lille, France},
series = {ICML'15}
}


@misc{li2020deepergcn,
    title={DeeperGCN: All You Need to Train Deeper GCNs},
    author={Guohao Li and Chenxin Xiong and Ali Thabet and Bernard Ghanem},
    year={2020},
    eprint={2006.07739},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@inproceedings{Kipf:2016tc,
  abstract = {We present a scalable approach for semi-supervised learning on graph-structured
data that is based on an efficient variant of convolutional neural networks which
operate directly on graphs. We motivate the choice of our convolutional architecture
via a localized first-order approximation of spectral graph convolutions.
Our model scales linearly in the number of graph edges and learns hidden layer
representations that encode both local graph structure and features of nodes. In
a number of experiments on citation networks and on a knowledge graph dataset
we demonstrate that our approach outperforms related methods by a significant
margin.},
  added-at = {2020-07-15T00:50:01.000+0200},
  author = {Kipf, Thomas N. and Welling, Max},
  biburl = {https://www.bibsonomy.org/bibtex/271ee5be8cafc25d7a3869bcb49fc5c3c/twagener},
  booktitle = {Proceedings of the 5th International Conference on Learning Representations},
  interhash = {54b65044b71f10c31476ed76422ab85d},
  intrahash = {71ee5be8cafc25d7a3869bcb49fc5c3c},
  keywords = {},
  location = {Palais des Congr{\`e}s Neptune, Toulon, France},
  series = {ICLR '17},
  timestamp = {2020-07-15T00:50:01.000+0200},
  title = {{Semi-Supervised Classification with Graph Convolutional Networks}},
  url = {https://openreview.net/forum?id=SJU4ayYgl},
  venue = {ICLR},
  year = 2017
}

@inproceedings{
GAT_vel,
title={Graph Attention Networks},
author={Petar Veličković and Guillem Cucurull and Arantxa Casanova and Adriana Romero and Pietro Liò and Yoshua Bengio},
booktitle={International Conference on Learning Representations},
year={2018},
url={https://openreview.net/forum?id=rJXMpikCZ},
}

@article{graphsage,
  added-at = {2020-01-17T13:30:25.000+0100},
  author = {Hamilton, Will and Ying, Zhitao and Leskovec, Jure},
  biburl = {https://www.bibsonomy.org/bibtex/2e8afa0739c75f78337a0e82484465564/denklu},
  interhash = {ad3fac0c6e1225815882f395bd58201d},
  intrahash = {e8afa0739c75f78337a0e82484465564},
  journal = {Advances in Neural Information Processing Systems},
  keywords = {},
  pages = {1024-1034},
  publisher = {Curran Associates, Inc.},
  timestamp = {2020-01-17T13:30:25.000+0100},
  title = {Inductive Representation Learning on Large Graphs},
  year = 2017
}


@misc{corso2020principal,
      title={Principal Neighbourhood Aggregation for Graph Nets}, 
      author={Gabriele Corso and Luca Cavalleri and Dominique Beaini and Pietro Liò and Petar Veličković},
      year={2020},
      eprint={2004.05718},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{beaini2020directional,
      title={Directional Graph Networks}, 
      author={Dominique Beaini and Saro Passaro and Vincent Létourneau and William L. Hamilton and Gabriele Corso and Pietro Liò},
      year={2020},
      eprint={2010.02863},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{JMLR:v15:srivastava14a,
  author  = {Nitish Srivastava and Geoffrey Hinton and Alex Krizhevsky and Ilya Sutskever and Ruslan Salakhutdinov},
  title   = {Dropout: A Simple Way to Prevent Neural Networks from Overfitting},
  journal = {Journal of Machine Learning Research},
  year    = {2014},
  volume  = {15},
  number  = {56},
  pages   = {1929-1958},
  url     = {http://jmlr.org/papers/v15/srivastava14a.html}
}

@misc{kukacka2017regularization,
      title={Regularization for Deep Learning: A Taxonomy}, 
      author={Jan Kukačka and Vladimir Golkov and Daniel Cremers},
      year={2017},
      eprint={1710.10686},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{dropout-hinton,
  author    = {Geoffrey E. Hinton and
               Nitish Srivastava and
               Alex Krizhevsky and
               Ilya Sutskever and
               Ruslan Salakhutdinov},
  title     = {Improving neural networks by preventing co-adaptation of feature detectors},
  journal   = {CoRR},
  volume    = {abs/1207.0580},
  year      = {2012},
  url       = {http://arxiv.org/abs/1207.0580},
  archivePrefix = {arXiv},
  eprint    = {1207.0580},
  timestamp = {Mon, 13 Aug 2018 16:46:10 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1207-0580.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{sohoni2019lowmemory,
      title={Low-Memory Neural Network Training: A Technical Report}, 
      author={Nimit Sharad Sohoni and Christopher Richard Aberger and Megan Leszczynski and Jian Zhang and Christopher Ré},
      year={2019},
      eprint={1904.10631},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{Bronstein_2017,
   title={Geometric Deep Learning: Going beyond Euclidean data},
   volume={34},
   ISSN={1558-0792},
   url={http://dx.doi.org/10.1109/MSP.2017.2693418},
   DOI={10.1109/msp.2017.2693418},
   number={4},
   journal={IEEE Signal Processing Magazine},
   publisher={Institute of Electrical and Electronics Engineers (IEEE)},
   author={Bronstein, Michael M. and Bruna, Joan and LeCun, Yann and Szlam, Arthur and Vandergheynst, Pierre},
   year={2017},
   month={Jul},
   pages={18–42}
}


@misc{chami2021machine,
      title={Machine Learning on Graphs: A Model and Comprehensive Taxonomy}, 
      author={Ines Chami and Sami Abu-El-Haija and Bryan Perozzi and Christopher Ré and Kevin Murphy},
      year={2021},
      eprint={2005.03675},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{bruna2014spectral,
      title={Spectral Networks and Locally Connected Networks on Graphs}, 
      author={Joan Bruna and Wojciech Zaremba and Arthur Szlam and Yann LeCun},
      year={2014},
      eprint={1312.6203},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}


@misc{duvenaud2015convolutional,
      title={Convolutional Networks on Graphs for Learning Molecular Fingerprints}, 
      author={David Duvenaud and Dougal Maclaurin and Jorge Aguilera-Iparraguirre and Rafael Gómez-Bombarelli and Timothy Hirzel and Alán Aspuru-Guzik and Ryan P. Adams},
      year={2015},
      eprint={1509.09292},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{henaff2015deep,
      title={Deep Convolutional Networks on Graph-Structured Data}, 
      author={Mikael Henaff and Joan Bruna and Yann LeCun},
      year={2015},
      eprint={1506.05163},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{monti2016geometric,
      title={Geometric deep learning on graphs and manifolds using mixture model CNNs}, 
      author={Federico Monti and Davide Boscaini and Jonathan Masci and Emanuele Rodolà and Jan Svoboda and Michael M. Bronstein},
      year={2016},
      eprint={1611.08402},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@inproceedings{liu-hgcn,
 author = {Liu, Qi and Nickel, Maximilian and Kiela, Douwe},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
 pages = {8230--8241},
 publisher = {Curran Associates, Inc.},
 title = {Hyperbolic Graph Neural Networks},
 url = {https://proceedings.neurips.cc/paper/2019/file/103303dd56a731e377d01f6a37badae3-Paper.pdf},
 volume = {32},
 year = {2019}
}

@inproceedings{chami-hgcn,
 author = {Chami, Ines and Ying, Zhitao and R\'{e}, Christopher and Leskovec, Jure},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
 pages = {4868--4879},
 publisher = {Curran Associates, Inc.},
 title = {Hyperbolic Graph Convolutional Neural Networks},
 url = {https://proceedings.neurips.cc/paper/2019/file/0415740eaa4d9decbc8da001d3fd805f-Paper.pdf},
 volume = {32},
 year = {2019}
}

@inproceedings{ganea-hyperbolic-NN,
 author = {Ganea, Octavian and Becigneul, Gary and Hofmann, Thomas},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {S. Bengio and H. Wallach and H. Larochelle and K. Grauman and N. Cesa-Bianchi and R. Garnett},
 pages = {5345--5355},
 publisher = {Curran Associates, Inc.},
 title = {Hyperbolic Neural Networks},
 url = {https://proceedings.neurips.cc/paper/2018/file/dbab2adc8f9d078009ee3fa810bea142-Paper.pdf},
 volume = {31},
 year = {2018}
}


@article{octonion-nns,
title = "Deep octonion networks",
journal = "Neurocomputing",
volume = "397",
pages = "179 - 191",
year = "2020",
issn = "0925-2312",
doi = "https://doi.org/10.1016/j.neucom.2020.02.053",
url = "http://www.sciencedirect.com/science/article/pii/S0925231220302435",
author = "Jiasong Wu and Ling Xu and Fuzhi Wu and Youyong Kong and Lotfi Senhadji and Huazhong Shu",
keywords = "Convolutional neural network, Complex, Quaternion, Octonion, Image classification",
abstract = "Deep learning is a hot research topic in the field of machine learning methods and applications. Real-value neural networks (Real NNs), especially deep real networks (DRNs), have been widely used in many research fields. In recent years, the deep complex networks (DCNs) and the deep quaternion networks (DQNs) have attracted more and more attentions. The octonion algebra, which is an extension of complex algebra and quaternion algebra, can provide more efficient and compact expressions. This paper constructs a general framework of deep octonion networks (DONs) and provides the main building blocks of DONs such as octonion convolution, octonion batch normalization and octonion weight initialization; DONs are then used in image classification tasks for CIFAR-10 and CIFAR-100 data sets. Compared with the DRNs, the DCNs, and the DQNs, the proposed DONs have better convergence and higher classification accuracy. The success of DONs is also explained by multi-task learning."
}


@InProceedings{pmlr-v97-wu19e,
  title = 	 {Simplifying Graph Convolutional Networks},
  author =       {Wu, Felix and Souza, Amauri and Zhang, Tianyi and Fifty, Christopher and Yu, Tao and Weinberger, Kilian},
  booktitle = 	 {Proceedings of the 36th International Conference on Machine Learning},
  pages = 	 {6861--6871},
  year = 	 {2019},
  editor = 	 {Kamalika Chaudhuri and Ruslan Salakhutdinov},
  volume = 	 {97},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {09--15 Jun},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v97/wu19e/wu19e.pdf},
  url = 	 {
http://proceedings.mlr.press/v97/wu19e.html
},
  abstract = 	 {Graph Convolutional Networks (GCNs) and their variants have experienced significant attention and have become the de facto methods for learning graph representations. GCNs derive inspiration primarily from recent deep learning approaches, and as a result, may inherit unnecessary complexity and redundant computation. In this paper, we reduce this excess complexity through successively removing nonlinearities and collapsing weight matrices between consecutive layers. We theoretically analyze the resulting linear model and show that it corresponds to a fixed low-pass filter followed by a linear classifier. Notably, our experimental evaluation demonstrates that these simplifications do not negatively impact accuracy in many downstream applications. Moreover, the resulting model scales to larger datasets, is naturally interpretable, and yields up to two orders of magnitude speedup over FastGCN.}
}


@inproceedings{
Zhao2020PairNorm:,
title={PairNorm: Tackling Oversmoothing in GNNs},
author={Lingxiao Zhao and Leman Akoglu},
booktitle={International Conference on Learning Representations},
year={2020},
url={https://openreview.net/forum?id=rkecl1rtwB}
}

@inproceedings{
savarese2018learning,
title={Learning Implicitly Recurrent {CNN}s Through Parameter Sharing},
author={Pedro Savarese and Michael Maire},
booktitle={International Conference on Learning Representations},
year={2019},
url={https://openreview.net/forum?id=rJgYxn09Fm},
}

@INPROCEEDINGS{low-rank-matrix-factorization,
  author={T. N. {Sainath} and B. {Kingsbury} and V. {Sindhwani} and E. {Arisoy} and B. {Ramabhadran}},
  booktitle={2013 IEEE International Conference on Acoustics, Speech and Signal Processing}, 
  title={Low-rank matrix factorization for Deep Neural Network training with high-dimensional output targets}, 
  year={2013},
  volume={},
  number={},
  pages={6655-6659},
  doi={10.1109/ICASSP.2013.6638949}}
  
  
@misc{hinton2015distilling,
  title={Distilling the Knowledge in a Neural Network}, 
  author={Geoffrey Hinton and Oriol Vinyals and Jeff Dean},
  year={2015},
  eprint={1503.02531},
  archivePrefix={arXiv},
  primaryClass={stat.ML}
}

@inproceedings{Hypernetworks,
title	= {HyperNetworks},
author	= {David Ha and Andrew Dai and Quoc V. Le},
year	= {2017},
URL	= {https://openreview.net/pdf?id=rkpACe1lx}
}

@InProceedings{Yang_2020_CVPR,
author = {Yang, Yiding and Qiu, Jiayan and Song, Mingli and Tao, Dacheng and Wang, Xinchao},
title = {Distilling Knowledge From Graph Convolutional Networks},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2020}
}


@misc{kong2020flag,
      title={FLAG: Adversarial Data Augmentation for Graph Neural Networks}, 
      author={Kezhi Kong and Guohao Li and Mucong Ding and Zuxuan Wu and Chen Zhu and Bernard Ghanem and Gavin Taylor and Tom Goldstein},
      year={2020},
      eprint={2010.09891},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{zhou2019graph,
      title={Graph Neural Networks: A Review of Methods and Applications}, 
      author={Jie Zhou and Ganqu Cui and Zhengyan Zhang and Cheng Yang and Zhiyuan Liu and Lifeng Wang and Changcheng Li and Maosong Sun},
      year={2019},
      eprint={1812.08434},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}


@inproceedings{glorot-init,
  added-at = {2019-05-29T00:00:00.000+0200},
  author = {Glorot, Xavier and Bengio, Yoshua},
  biburl = {https://www.bibsonomy.org/bibtex/221d2d1490c8404f823f1d36b294fce72/dblp},
  booktitle = {AISTATS},
  editor = {Teh, Yee Whye and Titterington, D. Mike},
  ee = {http://proceedings.mlr.press/v9/glorot10a.html},
  interhash = {4f45a520bb65b6045bd237963ffee0ed},
  intrahash = {21d2d1490c8404f823f1d36b294fce72},
  keywords = {dblp},
  pages = {249-256},
  publisher = {JMLR.org},
  series = {JMLR Proceedings},
  timestamp = {2019-05-30T11:50:49.000+0200},
  title = {Understanding the difficulty of training deep feedforward neural networks.},
  url = {http://dblp.uni-trier.de/db/journals/jmlr/jmlrp9.html#GlorotB10},
  volume = 9,
  year = 2010
}


@inproceedings{he-init,
author = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
title = {Delving Deep into Rectifiers: Surpassing Human-Level Performance on ImageNet Classification},
year = {2015},
isbn = {9781467383912},
publisher = {IEEE Computer Society},
address = {USA},
url = {https://doi.org/10.1109/ICCV.2015.123},
doi = {10.1109/ICCV.2015.123},
booktitle = {Proceedings of the 2015 IEEE International Conference on Computer Vision (ICCV)},
pages = {1026–1034},
numpages = {9},
series = {ICCV '15}
}

@misc{kingma2017adam,
      title={Adam: A Method for Stochastic Optimization}, 
      author={Diederik P. Kingma and Jimmy Ba},
      year={2017},
      eprint={1412.6980},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@incollection{pytorch,
title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
booktitle = {Advances in Neural Information Processing Systems 32},
editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
pages = {8024--8035},
year = {2019},
publisher = {Curran Associates, Inc.},
url = {https://bit.ly/3q9mtLS}
}


